CoFiDA-M: Concept-Aware Feature Modulation for Cross-Domain Adaptation with Image-Only Inference

Models for AI-based skin cancer screening suffer a severe performance drop when shifting from expert dermoscopic (source) images to consumer-grade clinical (target) images, hindering real-world deployment. Existing domain adaptation methods often ignore crucial semantic invariants, such as clinical concepts. While new foundation models like MONET can provide this semantic information as dense, probabilistic scores, this metadata is unavailable at test time, creating a deployment paradox for practical image-only screening tools. We address this gap by proposing CoFiDA-M, a privileged information framework that learns from concepts at training time but deploys as an image-only model. Our method trains a teacher network that uses MONET concept probabilities to guide a FiLM modulator, transforming visual features into a semantically ``edited" feature space. A lightweight, image-only student is then trained to reproduce this edited representation, not just the teacher's final predictions. This distillation ``bakes" the clinical reasoning into the student's weights. On a challenging multi-dataset benchmark, our image-only student significantly outperforms state-of-the-art approaches, especially in melanoma recall. Our work provides a practical and generalizable framework for leveraging noisy, probabilistic metadata as privileged information, demonstrating strong cross-dataset robustness and potential for real-world deployment beyond dermatology. Implementation code is available at: https://github.com/mmu-dermatology-research/CoFiDA.git

==> AUROC_cli.tex <==
\begingroup
\sisetup{
  separate-uncertainty = true,
  table-number-alignment = center,
  detect-weight = true,
  detect-family = true
}
\begin{table}[h]
\centering
\scriptsize
\caption{AUROC (\%) mean $\pm$ std over 3 seeds with macro-averages. Top: \textbf{Dermoscopic} (Md, MIDd, D7d, HAM). Bottom: \textbf{Clinical} (Mc, MIDc, D7c, Fitz).}
\label{tab:auroc_derm_and_clinic_with_avg}
\renewcommand{\arraystretch}{1.05}

% ---------- (a) Dermoscopic ----------
\textbf{(a) Dermoscopic}\\
\resizebox{\linewidth}{!}{%
\begin{tabular}{
  l
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2]
}
\toprule
\textbf{Setting / Method} & {\textbf{Md}} & {\textbf{MIDd}} & {\textbf{D7d}} & {\textbf{HAM}} & {\textbf{Avg}} \\
\midrule
\multicolumn{6}{l}{\textbf{Classical}} \\
DANN        & \num{78.37 \pm 0.01} & \num{72.29 \pm 0.18} & \num{69.40 \pm 0.17} & \num{72.09 \pm 0.16} & 73.04 \\
DeepCoral   & \num{79.20 \pm 0.24} & \num{69.55 \pm 0.19} & \num{52.39 \pm 0.31} & \num{76.87 \pm 0.22} & 69.50 \\
MMD         & \num{78.23 \pm 0.10} & \num{75.83 \pm 0.10} & \num{62.15 \pm 0.05} & \num{80.10 \pm 0.21} & 74.08 \\
MeanTeacher & \num{62.06 \pm 0.26} & \num{45.34 \pm 0.13} & \num{51.22 \pm 0.20} & \num{65.27 \pm 0.13} & 55.97 \\
\midrule
\multicolumn{6}{l}{\shortstack[l]{\textbf{Modern}\\\textbf{Source Free}}} \\
SHOT++      & \num{65.17 \pm 0.22} & \num{52.57 \pm 0.08} & \num{62.19 \pm 0.24} & \num{61.45 \pm 0.21} & 60.35 \\
DINE        & \num{70.32 \pm 0.19} & \num{71.80 \pm 0.20} & \num{65.39 \pm 0.12} & \num{79.81 \pm 0.18} & 71.83 \\
SFDA        & \num{58.49 \pm 0.11} & \num{55.76 \pm 0.16} & \num{55.95 \pm 0.03} & \num{54.12 \pm 0.19} & 56.08 \\
\midrule
\multicolumn{6}{l}{\shortstack[l]{\textbf{Modern}\\\textbf{Test Time}}} \\
CoTTA       & \num{62.43 \pm 0.24} & \num{53.60 \pm 0.22} & \num{55.79 \pm 0.01} & \num{54.61 \pm 0.17} & 56.61 \\
TENT        & \num{80.21 \pm 0.16} & \num{65.30 \pm 0.04} & \num{70.08 \pm 0.19} & \num{63.21 \pm 0.22} & 69.70 \\
WoC         & \num{66.29 \pm 0.21} & \num{58.19 \pm 0.09} & \num{61.05 \pm 0.20} & \num{54.71 \pm 0.14} & 60.06 \\
\midrule
\multicolumn{6}{l}{\textbf{Multimodal}} \\
BLIP        & \num{73.46 \pm 0.20} & \num{69.75 \pm 0.18} & \num{59.41 \pm 0.22} & \num{59.12 \pm 0.23} & 65.43 \\
MIMO        & \num{75.50 \pm 0.19} & \num{61.15 \pm 0.21} & \num{49.22 \pm 0.06} & \num{61.05 \pm 0.20} & 61.73 \\
\bottomrule
Source Only & \num{84.67 \pm 0.06} & \num{65.94 \pm 0.03} & \num{54.76 \pm 0.02} & \num{74.48 \pm 0.01} & 69.96 \\
Ours (CoFIDA-M)  & \num{89.70 \pm 0.09} & \num{76.15 \pm 0.07} & \num{61.69 \pm 0.07} & \num{78.45 \pm 0.05} & 76.50 \\
\bottomrule
\end{tabular}%
}

\vspace{6pt}

% ---------- (b) Clinical ----------
\textbf{(b) Clinical}\\
\resizebox{\linewidth}{!}{%
\begin{tabular}{
  l
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2]
}
\toprule
\textbf{Setting / Method} & {\textbf{Mc}} & {\textbf{MIDc}} & {\textbf{D7c}} & {\textbf{Fitz}} & {\textbf{Avg}} \\
\midrule
\multicolumn{6}{l}{\textbf{Classical}} \\
DANN         & \num{76.81 \pm 0.02} & \num{56.43 \pm 0.11} & \num{43.84 \pm 0.05} & \num{55.23 \pm 0.04} & 58.08 \\
DeepCoral    & \num{77.30 \pm 0.16} & \num{50.41 \pm 0.07} & \num{49.37 \pm 0.19} & \num{48.76 \pm 0.06} & 56.46 \\
MMD          & \num{79.58 \pm 0.14} & \num{52.25 \pm 0.05} & \num{46.74 \pm 0.16} & \num{56.10 \pm 0.08} & 58.67 \\
MeanTeacher  & \num{53.08 \pm 0.20} & \num{48.81 \pm 0.05} & \num{47.46 \pm 0.09} & \num{46.30 \pm 0.16} & 48.91 \\
\midrule
\multicolumn{6}{l}{\shortstack[l]{\textbf{Modern}\\\textbf{Source Free}}} \\
SHOT++       & \num{55.88 \pm 0.03} & \num{57.39 \pm 0.02} & \num{51.10 \pm 0.20} & \num{39.01 \pm 0.12} & 50.84 \\
DINE         & \num{66.54 \pm 0.15} & \num{52.93 \pm 0.25} & \num{41.22 \pm 0.11} & \num{56.94 \pm 0.07} & 54.41 \\
SFDA         & \num{44.91 \pm 0.12} & \num{47.27 \pm 0.05} & \num{45.39 \pm 0.16} & \num{51.42 \pm 0.13} & 47.25 \\
\midrule
\multicolumn{6}{l}{\shortstack[l]{\textbf{Modern}\\\textbf{Test Time}}} \\
CoTTA        & \num{51.99 \pm 0.14} & \num{50.55 \pm 0.15} & \num{53.71 \pm 0.08} & \num{52.75 \pm 0.09} & 52.25 \\
TENT         & \num{81.76 \pm 0.11} & \num{55.09 \pm 0.17} & \num{55.78 \pm 0.15} & \num{56.63 \pm 0.14} & 62.32 \\
WoC          & \num{49.76 \pm 0.13} & \num{43.57 \pm 0.16} & \num{60.73 \pm 0.19} & \num{41.87 \pm 0.02} & 48.98 \\
\midrule
\multicolumn{6}{l}{\textbf{Multimodal}} \\
BLIP         & \num{73.57 \pm 0.18} & \num{63.39 \pm 0.16} & \num{54.56 \pm 0.17} & \num{57.28 \pm 0.15} & 62.20 \\
MIMO         & \num{59.49 \pm 0.10} & \num{51.14 \pm 0.14} & \num{58.29 \pm 0.21} & \num{56.06 \pm 0.06} & 56.25 \\
\bottomrule
Source Only  & \num{75.02 \pm 0.04} & \num{51.51 \pm 0.02} & \num{52.85 \pm 0.08} & \num{54.20 \pm 0.01} & 58.39 \\
Ours (CoFIDA-M) & \num{83.94 \pm 0.01} & \num{69.67 \pm 0.04} & \num{50.48 \pm 0.26} & \num{65.91 \pm 0.09} & 67.50 \\
\bottomrule
\end{tabular}%
}
\end{table}
\endgroup


==> AUROC_der.tex <==
\begingroup
\sisetup{
  separate-uncertainty = true,
  table-number-alignment = center,
  detect-weight = true,
  detect-family = true
}
\begin{table}[H]
\centering
\scriptsize
\caption{Dermoscopic AUROC (\%) mean $\pm$ std over 3 seeds. \textbf{Avg} is the macro-average across Md, MIDd, D7d, and HAM.}
\label{tab:auroc_derm_with_avg}
\renewcommand{\arraystretch}{1.05}
\resizebox{\linewidth}{!}{%
\begin{tabular}{
  l
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2(2)]
  S[table-format=2.2] % Avg (number only)
}
\toprule
\textbf{Setting / Method} & {\textbf{Md}} & {\textbf{MIDd}} & {\textbf{D7d}} & {\textbf{HAM}} & {\textbf{Avg}} \\
\midrule
\multicolumn{6}{l}{\textbf{Classical}} \\
DANN        & \num{78.37 \pm 0.01} & \num{72.29 \pm 0.18} & \num{69.40 \pm 0.17} & \num{72.09 \pm 0.16} & 73.04 \\
DeepCoral   & \num{79.20 \pm 0.24} & \num{69.55 \pm 0.19} & \num{52.39 \pm 0.31} & \num{76.87 \pm 0.22} & 69.50 \\
MMD         & \num{78.23 \pm 0.10} & \num{75.83 \pm 0.10} & \num{62.15 \pm 0.05} & \num{80.10 \pm 0.21} & 74.08 \\
MeanTeacher & \num{62.06 \pm 0.26} & \num{45.34 \pm 0.13} & \num{51.22 \pm 0.20} & \num{65.27 \pm 0.13} & 55.97 \\
\midrule
\multicolumn{6}{l}{\shortstack[l]{\textbf{Modern}\\\textbf{Source Free}}} \\
SHOT++      & \num{65.17 \pm 0.22} & \num{52.57 \pm 0.08} & \num{62.19 \pm 0.24} & \num{61.45 \pm 0.21} & 60.35 \\
DINE        & \num{70.32 \pm 0.19} & \num{71.80 \pm 0.20} & \num{65.39 \pm 0.12} & \num{79.81 \pm 0.18} & 71.83 \\
SFDA        & \num{58.49 \pm 0.11} & \num{55.76 \pm 0.16} & \num{55.95 \pm 0.03} & \num{54.12 \pm 0.19} & 56.08 \\
\midrule
\multicolumn{6}{l}{\shortstack[l]{\textbf{Modern}\\\textbf{Test Time}}} \\
CoTTA       & \num{62.43 \pm 0.24} & \num{53.60 \pm 0.22} & \num{55.79 \pm 0.01} & \num{54.61 \pm 0.17} & 56.61 \\
TENT        & \num{80.21 \pm 0.16} & \num{65.30 \pm 0.04} & \num{70.08 \pm 0.19} & \num{63.21 \pm 0.22} & 69.70 \\
WoC         & \num{66.29 \pm 0.21} & \num{58.19 \pm 0.09} & \num{61.05 \pm 0.20} & \num{54.71 \pm 0.14} & 60.06 \\
\midrule
\multicolumn{6}{l}{\textbf{Multimodal}} \\
BLIP        & \num{73.46 \pm 0.20} & \num{69.75 \pm 0.18} & \num{59.41 \pm 0.22} & \num{59.12 \pm 0.23} & 65.43 \\
MIMO        & \num{75.50 \pm 0.19} & \num{61.15 \pm 0.21} & \num{49.22 \pm 0.06} & \num{61.05 \pm 0.20} & 61.73 \\
\bottomrule
Source Only & \num{84.67 \pm 0.06} & \num{65.94 \pm 0.03} & \num{54.76 \pm 0.02} & \num{74.48 \pm 0.01} & 69.96 \\
Ours (CoFIDA-M)  & \num{89.70 \pm 0.09} & \num{76.15 \pm 0.07} & \num{61.69 \pm 0.07} & \num{78.45 \pm 0.05} & 76.50 \\
\bottomrule
\end{tabular}%
}
\end{table}
\endgroup


==> ablation.tex <==
\sisetup{
  round-mode          = places,
  round-precision     = 2,
  table-number-alignment = center,
  detect-weight       = true,
  detect-inline-weight= math
}

% ---------------- Table (Teacher MONET sanity, updated) ----------------
\begin{table}[H]
\centering
\caption{Teacher ablations testing whether MONET carries signal. All rows use image\,+\,MONET at test. “Shuffle” permutes MONET within a batch; “Random” replaces MONET with noise. AUROC (↑), BAcc (↑), ECE (↓), latency (ms/img). \textbf{Protocol:} teacher models are evaluated with \emph{EMA} weights (shadow) if present; student/backbone use non-EMA model weights. Checkpoints selected by the same criterion across rows (fixed run); no test-time augmentation; input resized to $288{\times}288$, ImageNet normalisation; MONET vectors taken from the MILK10k CSV by matching \texttt{lesion\_id} and dataset \texttt{image\_type}; BAcc computed at $p{=}0.5$; ECE with 15 equal-width bins; single seed (42); latency measured end-to-end on the same machine.}

\label{tab:teacher_monet_sanity}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l l
                S[table-format=1.4]  % AUROC
                S[table-format=1.4]  % BAcc
                S[table-format=1.4]  % ECE
                S[table-format=2.2]  % ms/img
               }
\toprule
\multicolumn{2}{l}{\textbf{Model / Setting}} & {\textbf{AUROC}\,\(\uparrow\)} & {\textbf{BAcc}\,\(\uparrow\)} & {\textbf{ECE}\,\(\downarrow\)} & {\textbf{ms/img}\,\(\downarrow\)} \\
\midrule
\multicolumn{6}{l}{\textit{Clinic}}\\
Teacher & Real    & {\bfseries 0.7864} & 0.7327 & 0.8914 & 4.80 \\
        & Shuffle & 0.6069             & 0.5029 & 0.8765 & 3.77 \\
        & Random  & 0.6672             & 0.5363 & 0.8837 & 3.78 \\
\addlinespace[1ex]
\multicolumn{6}{l}{\textit{Dermoscopic}}\\
Teacher & Real    & {\bfseries 0.7936} & 0.6808 & 0.8079 & 3.64 \\
        & Shuffle & 0.6638             & 0.5904 & 0.8124 & 3.70 \\
        & Random  & 0.7066             & 0.6017 & 0.7974 & 3.68 \\
\bottomrule
\end{tabular}
\end{table}



\begin{comment}
    

\sisetup{
  round-mode=places,
  round-precision=4,
  table-number-alignment=center,
  detect-weight=true, detect-inline-weight=math
}
\newcommand{\bestnum}[1]{{\bfseries #1}} % safe for S columns

\begin{table}[H]
\centering
\caption{Image-only student (CoFiDA-M, distilled) evaluated across eight datasets. 
Reported: balanced accuracy (BAcc) \(\uparrow\), accuracy \(\uparrow\), calibration error (ECE) \(\downarrow\), latency (ms/img) \(\downarrow\).}
\label{tab:student_ablation}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l
                S[table-format=1.4]  % BAcc
                S[table-format=1.4]  % Acc
                S[table-format=1.4]  % ECE
                S[table-format=2.2]  % ms/img
               }
\toprule
\textbf{Dataset} & {\textbf{BAcc}} & {\textbf{Acc}} & {\textbf{ECE}} & {\textbf{ms/img}} \\
\midrule
Mc     & 0.7974 & 0.7424 & 0.8941 &  3.93 \\
Md     & 0.7809 & 0.7405 & 0.8757 &  3.22 \\
MIDc   & 0.6409 & 0.6427 & 0.8010 & 43.68 \\
MIDd   & 0.7035 & 0.7202 & 0.8758 & 43.85 \\
HAM & 0.5561 & 0.2668 & 0.8466 &  5.42 \\
Fitz   & 0.6414 & 0.7109 & 0.8328 &  3.95 \\
D7c    & 0.4933 & 0.2742 & 0.7326 &  6.32 \\
D7d    & 0.4674 & 0.2618 & 0.7466 &  6.11 \\
\bottomrule
\end{tabular}
\end{table}}%

\end{comment}

%S1,S2,S3

\sisetup{round-mode=places,round-precision=4,table-number-alignment=center}
\newcommand{\na}{\textemdash} % placeholder for not-yet-run

\begin{table}[H]
\centering
\caption{Student ablation across datasets. S1: KD only; S2: KD+\(\mathcal{L}_u\); S3: S2+residual \(L_1\). 
Reported: BAcc \(\uparrow\), Acc \(\uparrow\), ECE \(\downarrow\), ms/img \(\downarrow\).}
\label{tab:student_s123}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l
    *{3}{S[table-format=1.4]}  % BAcc S1 S2 S3
    *{3}{S[table-format=1.4]}  % Acc  S1 S2 S3
    *{3}{S[table-format=1.4]}  % ECE  S1 S2 S3
    *{3}{S[table-format=2.2]}  % ms   S1 S2 S3
}
\toprule
        & \multicolumn{3}{c}{\textbf{BAcc} \(\uparrow\)} & \multicolumn{3}{c}{\textbf{Acc} \(\uparrow\)} &
          \multicolumn{3}{c}{\textbf{ECE} \(\downarrow\)} & \multicolumn{3}{c}{\textbf{ms/img} \(\downarrow\)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
\textbf{Dataset} & \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S1} & \textbf{S2} & \textbf{S3} & \textbf{S1} & \textbf{S2} & \textbf{S3} \\
\midrule
Mc    & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7974 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7424 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.8941 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} &  3.93 \\
Md    & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7809 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7405 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.8757 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} &  3.22 \\
MIDc  & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.6409 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.6427 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.8010 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 43.68 \\
MIDd  & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7035 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7202 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.8758 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 43.85 \\
HAM   & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.5561 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.2668 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.8466 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} &  5.42 \\
Fitz  & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.6414 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7109 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.8328 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} &  3.95 \\
D7c   & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.4933 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.2742 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7326 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} &  6.32 \\
D7d   & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.4674 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.2618 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} & 0.7466 & \multicolumn{1}{c}{\na} & \multicolumn{1}{c}{\na} &  6.11 \\
\bottomrule
\end{tabular}
\end{table}






\newcommand{\cmark}{\ding{51}}   % ✓
\newcommand{\xmark}{\ding{55}}   % ✗
\newcommand{\dash}{\textemdash}  % —
\sisetup{
  round-mode=places, round-precision=2,
  detect-weight=true, detect-family=true,
  table-number-alignment=center
}

% ----- table in your paper -----
\begin{table*}[h]
\centering
\caption{Model variants without AUPRC. “Concepts at test” indicates whether MONET is required at inference. 
KD = logits distillation; $\mathcal{L}_u$ = edited-feature alignment; Residual L1 = sparsity on the student edit.}
\label{tab:summary_variants_no_auprc}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{
  l
  c c c c
  S[table-format=1.4]  % AUROC
  S[table-format=1.4]  % Acc
  S[table-format=1.4]  % ECE
  S[table-format=2.2]  % Params (M)
  S[table-format=2.2]  % ms/img
}
\toprule
\textbf{Model} & \textbf{Concepts at test} & \textbf{KD} & $\boldsymbol{\mathcal{L}_u}$ & \textbf{Residual L1} &
{\textbf{AUROC}\,$\uparrow$} & {\textbf{Acc}\,$\uparrow$} &
{\textbf{ECE}\,$\downarrow$} & {\textbf{Params (M)}} & {\textbf{ms/img}\,$\downarrow$} \\
\midrule
Image-only baseline & \xmark & \dash & \dash & \dash & ... & ... & ... & ... & ... \\
Teacher (FiLM)      & \cmark & \dash & \dash & \dash & ... & ... & ... & ... & ... \\
Student S1          & \xmark & \cmark& \dash & \dash & ... & ... & ... & ... & ... \\
Student S2          & \xmark & \cmark& \cmark& \dash & ... & ... & ... & ... & ... \\
Student S3          & \xmark & \cmark& \cmark& \cmark& ... & ... & ... & ... & ... \\
\bottomrule
\end{tabular}
\end{table*}
****************

visual abstract
\begin{figure}[h]
    \centering
\includegraphics[width=.47\textwidth]{sec/plot/vis_abstract.pdf}
  \caption{Left: Despite mixing dermoscopic and clinical data, conventional training yields poor separation at test time. Middle: During training, a confidence gated embedding module applies a FiLM edit that produces a well separated teacher feature space. Right: We distil this space into an image only student, enabling zero shot deployment on clinical images with no test time adaptation while preserving the teacher’s separation.}
    \label{vis_abstract}
\end{figure}

